A Highly Segmented Neutron Polarimeter for A1

A new neutron polarimeter for measuring the neutron's electric form factor was designed and constructed to complement the A1 spectrometer setup at the Mainz Microtron (MAMI). The design is based on a previous polarimeter with significant improvements to halve the error of the extracted form factor. A higher granularity of the polarimeter sections and a deeper first section on the one hand, and a faster readout employing Time-over-Threshold methods to measure the signal amplitudes combined with a high-precision FPGA-based TDC on the other hand will allow to achieve this goal. The performance of the new polarimeter during a first measurement campaign in 2019 using liquid hydrogen and deuterium targets will be discussed.

==> assembly.tex <==
The assembly of the detector modules, each consisting of a scintillator bar, two tapered light guides and two PMTs, is labor and skill intensive and requires several steps. In a first step, the tapered light guides are glued to the scintillator bar with optical cement (BC-600). To ensure a good optical coupling and a perfect alignment between bar and light guide, the gluing process has to be performed with the bars in a vertical position, in which the bars have to stay during the 24h hardening phase. Special adhesive frames have been developed and built for this purpose. After the first light guide is attached to the bar, the adhesive frame can be easily rotated to attach the second light guide. To ensure a good optical coupling, the process must be executed as uniformly as possible. Here, the quantity as well as the distribution of the optical cement on the joint surface play a crucial role: it has to be enough to allow for a homogeneous coverage along the entire surface, but excess glue should not contaminate the polished surfaces of the scintillator bars. Therefore a careful inspection during the adhesive process is mandatory.
With some add-on to the adhesive frame, the PMT can be glued to the light guides subsequently. In order to ensure an easy replacement of a PMT in case of malfunction or failure, the silicon elastomer Elastosil RT 601 was used for the optical coupling between light guide and PMT. Again, a 24h hardening phase is required.
The alignment of the PMT with respect to the light guide and the scintillator is the most crucial part of the whole gluing procedure. Even minor deviations can cause the PMT to detach unintentionally during the assembly of the detector.
Even if the procedure for manufacturing the scintillator modules is the same for both walls, different adhesive frames are required due to the different sizes of the bars. Up to five VETO or signal bars of the front wall can be aligned in the corresponding adhesive frame. For the various gluing steps, this frame can be turned over manually by two people. The larger bars of the rear wall are more complicated to handle due to their size and weight. Here, two bars are located in one adhesive frame. The construction allows for an easy rotation of the bars by a single person.
The scintillator modules are wrapped in one layer of reflective aluminum foil, followed by one layer of light-tight PVC foil.
